SCAN: A Spatial Context Attentive Network for Joint Multi-Agent Intent Prediction

Safe navigation of autonomous agents in human centric environments requires the ability to understand and predict motion of neighboring pedestrians. However, predicting pedestrian intent is a complex problem. Pedestrian motion is governed by complex social navigation norms, is dependent on neighbors' trajectories, and is multimodal in nature. In this work, we propose SCAN, a Spatial Context Attentive Network that can jointly predict socially-acceptable multiple future trajectories for all pedestrians in a scene. SCAN encodes the influence of spatially close neighbors using a novel spatial attention mechanism in a manner that relies on fewer assumptions, is parameter efficient, and is more interpretable compared to state-of-the-art spatial attention approaches. Through experiments on several datasets we demonstrate that our approach can also quantitatively outperform state of the art trajectory prediction methods in terms of accuracy of predicted intent.

==> fig_pred_len.tex <==
\begin{figure}
\centering
         \includegraphics[width=0.7\linewidth]{Figures/predlen.png}
         \caption{Change in ADE with prediction horizon length.}
        \label{fig:predlen}
\end{figure}


==> temporal_attention_mechanism.tex <==
In typical attention-based LSTM encoder-decoder frameworks, temporal attention is used to enable the decoder to variably \emph{attend} to the encoded hidden states. In this work, we attempt to adopt temporal attention mechanism to enable our model to attend to encoded \emph{spatial contexts}. This is similar to a pedestrian recollecting how to navigate through a certain crowd or evade a certain collision from past experiences. 
Therefore in our model, for every time step $t_p$ in the prediction time window, the decoder LSTM uses spatial attention to incorporate the spatial influence of neighbors on $p$ for generating a prediction for $p$. To be able to better understand the `spatial situation' at $t_p$ and arrive at a better prediction of intent at $t_p+1$, the LSTM \emph{temporally attends} to the spatially weighted hidden states in the input time window from $t_0$ to $T_{obs}$. The LSTM compares the current spatially weighted hidden state at $t_p$, $\tilde{h}^{p}_{t_p}$ to every $\tilde{h}^{p}_{t_s}$ for $t_s$ \in [$t_0$,$T_{obs}$] and assigns a score of similarity to each. The model then \emph{attends} more to hidden states that have been assigned a higher score in comparison to others. This is analogous to pedestrians learning to navigate safely through situations by learning from past experiences. 
This mechanism of attending variably to different time steps in the input time window is called temporal attention or soft attention~\cite{luong2015effective}. At each time step $t_p$ in the prediction sequence, the LSTM associated with pedestrian $p$ computes a \emph{context vector} as the weighted sum of (spatially-weighted) hidden states from the input time window. Each source hidden state from the encoder is assigned a \emph{score} (weight) to quantify its similarity to the target hidden state of the decoder. In our model, we use dot product to compute the \emph{score}. Therefore, the score assigned to an encoded spatially weighted hidden state would be maximum when the current spatially weighted hidden state of the decoder and the encoded spatially weighted hidden state being compared are `equal', which would mean that the spatial context experienced by the pedestrian at the current timestep is identical to that at the timestep from the encoder being compared. The soft attention context vector is then concatenated with the previous hidden state of the decoder, and is further input into the decoder LSTM. The output of the LSTM is then used to predict the next ($x$, $y$) coordinates for the pedestrian. This process is followed for all pedestrians in the frame at each timestep in the prediction time window.
%\begin{equation}
%    \mathbf{C}^p_{t_p} = \sum_{t_s=t_0}^{T_{obs}} %\alpha_{t_p}\tilde{h}_{t_s}^{p}
%\end{equation}

%The alignment vector $\alpha_{t_p}$, with length equal to the number of time steps in the input sequence, is derived by comparing the target spatially-weighted hidden state $\tilde{h}^{p}_{t_p}$ with each spatially-weighted hidden state $\tilde{h}_{t_s}^{p}$:
%\begin{equation}
%    \alpha_{t_p} = \mathbf{align}(\tilde{h}^{p}_{t_s},\tilde{h}^{p}_{t_p})
%\end{equation}
%
%\begin{equation}
 %   \mathbf{align}(~{h}^{p}_{t_s},~{h}^{p}_{t_p}) = \frac{\mathbf{exp}(\mathbf{score}(\tilde{h}^{p}_{t_s},\tilde{h}^{p}_{t_p})}{\sum_{s'}\mathbf{exp}(\mathbf{score}(\tilde{h}^{p}_{t_{s'}},\tilde{h}^{p}_{t_p})}
%\end{equation}
%where $\mathbf{score}$ is called \emph{content-based function} and is used to quantify the similarity of a source hidden state and a target hidden state. In our model, we use dot product to compute the $\mathbf{score}$. Therefore, the score assigned to an encoded spatially weighted hidden state would be maximum when the current spatially weighted hidden state of the decoder and the encoded spatially weighted hidden state being compared are `equal', which would mean that the spatial context experienced by the pedestrian at the current timestep is identical to that at the timestep from the encoder being compared. 
%The soft attention context vector $\mathbf{C}^{p}_{t_p}$ is computed at every $t_p$ \in [$T_{obs}+1, T_{pred}$]. At every time step, it is concatenated with the computed spatially weighted hidden state, $\tilde{h}^{p}_{t_{p}}$ and is further used to update the hidden state of the modular LSTM according to Equation \ref{eqn:lstm} and generate an intent prediction. A linear layer is used to embed the updated hidden state into a ($x$,$y$) prediction at $t_p$. 

